Tilting at windmills: Data augmentation for deep pose estimation does not help with occlusions

Occlusion degrades the performance of human pose estimation. In this paper, we introduce targeted keypoint and body part occlusion attacks. The effects of the attacks are systematically analyzed on the best performing methods. In addition, we propose occlusion specific data augmentation techniques against keypoint and part attacks. Our extensive experiments show that human pose estimation methods are not robust to occlusion and data augmentation does not solve the occlusion problems.

==> experiments.tex <==
%\section{Experiments}
%\subsubsection{Datasets}
%The experiments are performed on two of the main Human Pose Estimation datasets: COCO and MPII. The \textbf{COCO} dataset contains challenging imagery data with the unconstrained environment, different body scales, variety of human poses and occlusion patterns. This dataset contains over 200k images with 250k person instances labelled with 17 keypoints. Models are trained on COCO train2017 datasets, including 57k images and 150k person instances. The evaluation is done on val2017 set which contains 5k images. The \textbf{MPII} dataset consists of 40k person instances and each instance is labelled with 16 joints. The train set and validation sets includes 22k and 3k person instances respectively. The rest of the images are used for a test set of the competition. 
%\subsubsection{Evalutation metrics}
%For the evaluation of the models, Object Keypoint Similarity (OKS) for COCO and Percentage of Correct Keypoints
%(PCK) for MPII are used. 
%\subsubsection{Experimental setup}
%Training on COCO dataset was performed on 3 NVIDIA 1080TI GPUs for roughly 90 hours. The setup of training procedure was adopted by our baseline - HRNet\cite{HRNet}: Human detection boxes were extended to fit 4:3 aspect ratio, and then the boxes were cropped from the image, which is resized to a fixed size, $256 x 192$, or $384 x 288$. The data augmentations that are used in HRNet training include random rotation $\in [-45^o,45^o]$, random scale $\in [0.65, 1.35]$, random flipping and half-body augmentations. Adam optimizer \cite{adam} is used to train the network with the learning rate schedule following \cite{simple-baseline}, starting with $1e-3$ and reduced to $1e-4$ and $1e-5$ at 170th and 200th epochs respectively and the training is completed at the 210th epoch.
%\\\
%For MPII dataset, only the differences on training procedure are 256x256 input size and no usage of half-body augmentations.

\subsection{Targeted augmentations for single keypoint}
First, we checked the performance of 3 different augmentations which are applied on a single keypoint with the varying probability of 0.2 and 0.5: T. Blurring, T. Cutout and a combination of two of them. 
We obtained the boxes from Cascade RCNN detector which has ResNet50 backbone. We observe the highest improvement for T.Blurring and T.Cutout by $0.2\%$ when the varying probability is chosen as 0.5 (Table \ref{tab:abloation}). Other variants do not improve the performance.
% \begin{figure}[ht!]
% \centering
% {\includegraphics[width=.49\textwidth]{images/charts/detectors.pdf}}
% \caption{Performance of chosen augmentations for HRNet-32 on various detection backbones and ground truth boxes.}
% \label{fig:detector_performance}
% \end{figure}

\begin{figure}[ht!]
\centering
\subcaptionbox{Performance of chosen augmentations for HRNet-32 on various detection backbones and ground truth boxes. \label{fig:detector_performance}}{\includegraphics[width=.49\textwidth]{images/charts/detectors.pdf}}
\hfill
\subcaptionbox{Comparison between Baseline and T. Cutout (P}{\includegraphics[width=.49\columnwidth]{images/charts/radar_cutout.pdf}}
\caption{}
\end{figure}

\subsection{Targeted augmentations for multiple keypoints}
We applied 5 different multiple keypoints augmentation methods: part level T. Blurring, T. Cutout, a combination of both them; T. PartMix and  random Targeted Multikeypoint variant T. Blurring and T. Cutout with a maximum of 5 keypoints.
To demonstrate the effect of each augmentation, we apply them with a probability of 0.2 and 0.5. In addition, the effect of removing the labels of the occluded keypoint is also investigated as \textit{removal} column in  Table \ref{tab:abloation}.
\\\
In the bottom part of Table \ref{tab:abloation}, T. Cutout and T. PartMix show 0.2\% and 0.1\% improvements respectively. In all the variants of T. Blurring, small degradation or no improvement is observed. The combination of part level variants of T. Cutout and T. Blurring indicate some decreases of the performance (removal with probability of 0.2 and 0.5) and do not improve in non-removal configuration. Random T. Multikeypoint decreases the performance by 0.4\%. For all the multiple keypoint augmentations, it is important to keep the occluded keypoints since they bring better or on a par result with the baseline.
\begin{table*}[t]
  \centering
  \begin{tabular}{l c c c c c c c c c c c}
    % \toprule
    & \multicolumn{7}{r}{\small{\textbf{Evaluation results}}} \\
    \cmidrule(r){5-12}
    {\small\textit{Augmentation}}
    & {\small \textit{level}}
    & {\small \textit{remove}}
    & {\small \textit{p}}
    & {\small \textit{Head}}
    & {\small \textit{Shoulder}}
    & {\small \textit{Elbow}}
    & {\small \textit{Wrist}}
    & {\small \textit{Hip}}
     & {\small \textit{Knee}}
    & {\small \textit{Ankle}}  & {\small \textit{\textbf{Total}}}\\
    % Hea Sho Elb Wri Hip Kne Ank Total
    \midrule \midrule
    {Baseline}&-& - & - & 97.1 & 95.9 & 90.4 &   86.4 & 89.1 & 87.2 & 83.3 & 90.3\\
    % \midrule
    {T. Blurring} & k & \xmark &0.5 & 97.3 & 95.9 & 90.5 & 86.2 & 89.2 & 86.4 & 83.1 & 90.3 \\
    % \midrule
    T. Cutout & p & \xmark& 0.5 & 97.2&  96.3 & 90.7 & 86.7 & 89.4 & 86.7 & 83.3 & \textbf{90.5}\\
    % \midrule
    {T. PartMix} &- &\xmark & 0.5 & 97.4 & 96.2 & 91.0 & 86.8 & 89.2 & 86.7 & 83.0 & \textbf{90.5}\\
    % \bottomrule
  \end{tabular}
  \caption{Results on MPII dataset. \jvg{Read 'booktabs.pdf', no horizontal lines in tables, except top and bottom} Keypoint T. Blurring obtains on a par with the baseline, yet part level T. Cutout and T. PartMix increase the performance.}
  \label{tab:mpii_results}
\end{table*}
\subsection{What is the effect of object detector on human pose estimation?}
Aforementioned in Section \ref{method}, Top-Down type pose estimators use an object detection algorithm to obtain human instances. Therefore, the performance of the pose estimation considerably depends on the detection performance. 
Starting from this section, we use only T. keypoint Blurring, T. part Cutout and T. PartMix methods for further analysis as they are most promising augmentations.
In this section, we evaluate the pose estimation performances of HRNet baseline and HRNet with our augmentation methods with 2 2-stage detectors, Faster RCNN with XCeption 101 backbone and Cascade RCNN; 2 single-stage detectors, RetinaNet and EfficientDet D7; and by using ground truth boxes of human instances (Figure \ref{fig:detector_performance}). 

All augmentations demonstrate a notable improvements using Ground truth bounding boxes by $0.2\%$  for T. Blurring and T. PartMix, and $0.4\%$ for T. Cutout. All our augmentation methods obtain better result with Cascade RCNN and RetinaNet $0.1-0.2\%$ depending on the augmentation. 
With EfficientDet D7 detector, our augmentations result in similar to baseline except $0.1\%$ improvement by T. PartMix. 
For Faster-RCNN, T. Blurring shows $0.2\%$ increase, yet T. Cutout degrades the performance by $0.1\%$. 
\subsection{Performance on MPII}
We also tested our data augmentation methods on MPII dataset (Table \ref{tab:mpii_results}).
If we check the total contribution of our augmentation, T. keypoint Blurring result in on a par with baseline, yet T. part Cutout and T. PartMix increase the performance by $0.2\%$ for the metric PCK@0.5. 
The largest improvement per keypoint is observed for elbows by $0.6\%$ and wrists by $0.3\%$, with the degradation on knees ankles by $0.4\%$ and $0.2\%$ respectively. 

\subsection{How occlusion robust is data augmentation?}
The analysis of the robustness of the baseline and the proposed augmentations to the occlusion techniques which are introduced in Section~\ref{problem} can be seen in Figure~\ref{fig:ressilience_table}. The analysis is done on COCO dataset and the results are shown as mAP score of all keypoints.
We can clearly see that training with the keypoint level T. Blurring makes the system more robust against very same method, but there is no significant improvement for the other keypoint level occlusions. 
For the part level augmentations, there is a clear improvement against part level blackout and meanout occlusions in comparison to baseline. 
Specifically, T. PartMix has almost no advantages for keypoint level occlusions, however it significantly improves part level methods about $0.5\%$ for blackout and meanout part level occlusions.
T. Cutout shows notable drop in the performance for the keypoint level meanout, and a significant increase for methods for part level blurring and meanout by $0.3\%$ and $0.5\%$ respectively. 
% \begin{figure}[ht!]
% \centering
% \subcaptionbox{Comparison between Baseline and T. Blurring (K)}{\includegraphics[width=.49\columnwidth]{images/charts/radar_blurring.pdf}}
% \hfill
% \subcaptionbox{Comparison between Baseline and T. Cutout (P}{\includegraphics[width=.49\columnwidth]{images/charts/radar_cutout.pdf}}
% \subcaptionbox{Comparison between Baseline and T. PartMix}{\includegraphics[width=.49\columnwidth]{images/charts/radar_partmix.pdf}}
% \caption{Comparison for average loss in performance across occlusion attacks for proposed data augmentations.}
% \end{figure}

\begin{figure}[ht!]
\centering
\subcaptionbox{Comparison of chosen augmentation on keypoint level attacks.}{\includegraphics[width=.49\columnwidth]{images/charts/radar_keypoint.pdf}}
\hfill
\subcaptionbox{Comparison of chosen augmentation on part level attacks. }{\includegraphics[width=.49\columnwidth]{images/charts/radar_part.pdf}}

\end{figure}


